Self-Enhanced GNN: Improving Graph Neural Networks Using Model Outputs

Graph neural networks (GNNs) have received much attention recently because of their excellent performance on graph-based tasks. However, existing research on GNNs focuses on designing more effective models without considering much about the quality of the input data. In this paper, we propose self-enhanced GNN (SEG), which improves the quality of the input data using the outputs of existing GNN models for better performance on semi-supervised node classification. As graph data consist of both topology and node labels, we improve input data quality from both perspectives. For topology, we observe that higher classification accuracy can be achieved when the ratio of inter-class edges (connecting nodes from different classes) is low and propose topology update to remove inter-class edges and add intra-class edges. For node labels, we propose training node augmentation, which enlarges the training set using the labels predicted by existing GNN models. SEG is a general framework that can be easily combined with existing GNN models. Experimental results validate that SEG consistently improves the performance of well-known GNN models such as GCN, GAT and SGC across different datasets.

==> 2_preliminaries.tex <==
% !TEX root = ./main.tex

\section{Preliminaries}

\textbf{Semi-Supervised Node Classification} 
\quad In space \(\mathbb{V}\), nodes are assigned with a label from \(1\) to \(C\), where \(C\) is the total number of classes. \(\M{Y}\) is the class assignment vector for all the nodes in \(\mathbb{V}\). The objective of semi-supervised node classification is to utilize the labeled nodes to learn a mapping function \(f:\mathbb{V} \rightarrow \left\{1,\ldots, C\right\}\) that can generalize to predict the unlabeled nodes in space \(\mathbb{V}\). In transductive graph semi-supervised node classification setting, the nodes features \(\M{X}\) and the graph structure \(A\) of a graph \(\M{G(V,E)}\) are given.  \\
\textbf{Graph Neural Network}
\quad The graph convolution is proposed by AAA, from the spectral graph analysis perspective. \\
\textbf{Graph Topology}
\quad Edges play an extreme role in graph node classification task.\\
\textbf{Noisy Label Training}
\quad The goal of noisy label training is to train a robust model on a training set which may contains some nodes with false labels.



==> 6_related_work.tex <==
% !TEX root = ./main.tex
\section{Related Work}	\label{sec:related}

\vspace{1mm}

\noindent\textbf{GNN models.}  Many GNN models have been proposed in recent years, including GCN~\cite{kipf2017semi}, GAT~\cite{velickovic2018graph}, SGC~\cite{felix2019simplifying}, GraphSAGE~\cite{hamilton2017inductive}, Geom-GCN~\cite{pei2020geomgcn}, GGNN~\cite{li2015gated}, JK-Net~\cite{xu2018representation}, ChebNet~\cite{defferrard2016convolutional}, Highway GNN~\cite{zilly2017recurrent} and MoNet~\cite{monti2017geometric}. These works focus on improving the performance of a task, e.g., the prediction accuracy of node classification, comparing with prior methods. In contrast, our method, self-enhanced GNN, aims to improve the quality of the input data. By providing data with higher quality, self-enhanced GNN provides a general framework that can be easily applied on existing GNN models to further improve their performance. 

To the best of our knowledge, our work is most related to \citet{chen2019measuring} and \citet{li2018deeper}. \citet{chen2019measuring} observed that the performance of GNN models usually degrades when using more than 2 layers due to local smoothing and proposed to remove/add edges in a graph to mitigate the over-smoothing problem of GNN models. In contrast, we come from the perspective of data quality and observe that lower noise ratio leads to higher classification accuracy. In addition, we provide theoretical analysis to show that adding/removing edges can reduce noise ratio if the performance of a model is good enough. The idea of enlarging the training set  with co-training and self-training was proposed in~\cite{li2018deeper}, which corresponds to the single-model case of our training node augmentation algorithm. However, as we have shown in our analysis and profiling results in Section~\ref{tna:opt}, using the diversity of multiple models and explicitly balancing the classes in the training set are crucial for performance. In fact, the results reported in~\cite{li2018deeper} also show that the performance of GNN (e.g., GCN) actually degrades in many cases when applying co-training and self-training with a single model.


%\citet{li2018deeper} enlarges the training set with co-training and self-training, which corresponds to the single-model case of our training node augmentation algorithm. As we have shown in our analysis and experiments, using the diversity of multiple models and explicitly balancing the classes in the training set is crucial for performance.  

\vspace{1mm}


\noindent\textbf{Noisy label training.} Self-enhanced GNN is partly motivated by noisy label training, which aims at learning good models from data with noisy labels, i.e., a large number of training samples come with wrong labels. Representative work along this line include Decoupling~\cite{malach2017decoupling}, MentorNet~\cite{jiang2017mentornet}, Noisy Cross-Validation~\cite{chen2019ncv} and Co-teaching~\cite{han2018co}. These works focus on how to select samples with possibly correct labels from a noisy dataset to conduct model training, and our multi-model sample selection method is motivated by these works. However, as GNNs work on graph data, self-enhanced GNN handles not only noise in labels but also noise in the graph structure (i.e., inter-class edges) with topology update. Given the excellent performance of GNNs on graph data, a potential direction is to apply self-enhanced GNN to noisy label training. With the assumption that samples with similar features are likely to share the same label, a similarity graph (e.g., a $k$-nearest-neighbor graph based on image descriptors) can be constructed on a noisy dataset and noisy label training can be modeled as a semi-supervised node classification problem on graphs.

